Event-triggered output feedback stabilization via dynamic high-gain scaling

-This work addresses output feedback stabilization via event triggered output feedback. In the first part of the paper, linear systems are considered, whereas the second part shows that a dynamic event triggered output feedback control law can achieve feedback stabilization of the origin for a class of nonlinear systems by employing dynamic high-gain techniques.

==> newcommands_mathGeneral.tex <==
\DeclareMathOperator{\diag}{diag}

%- inverse
\newcommand{\inv}[1]{(#1)^{-1}}

%- pour justifier à droite une ligne dans l'environnement align
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Pour les systemes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\temp}{a}
%- Version non numerotee
\makeatletter
\newcommand{\@syst}[1]{%
\[
\left\{
\begin{aligned}
#1
\end{aligned}
\right.
\]
}
\newenvironment{syst}{\collect@body\@syst}{\global\@ignoretrue}

%- Version numerotee
\newcommand{\@systn}[1]{%
\begin{equation}
\left\{
\begin{aligned}
#1
\end{aligned}
\right.
\end{equation}
}
\newenvironment{systn}{\collect@body\@systn}{\global\@ignoretrue}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ensembles de nombres
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\LL}{{\mathbb{L}}}
\newcommand{\RR}{{\mathbb{R}}}
\newcommand{\NN}{{\mathbb{N}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fractions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%- displaystyle
\newcommand{\fracDisplay}[2]{\displaystyle \frac{#1}{#2}}             
%- dérivées partielles
\newcommand{\dd}[2]{\displaystyle \fracDisplay{\partial #1}{\partial #2}}

%%%%%%%%%%%%
%- norm
\newcommand{\norm}[1]{\left\| #1 \right\|}
